What really matters for person re-identification? A Mixture-of-Experts Framework for Semantic Attribute Importance

State-of-the-art person re-identification methods achieve impressive accuracy but remain largely opaque, leaving open the question: which high-level semantic attributes do these models actually rely on? We propose MoSAIC-ReID, a Mixture-of-Experts framework that systematically quantifies the importance of pedestrian attributes for re-identification. Our approach uses LoRA-based experts, each linked to a single attribute, and an oracle router that enables controlled attribution analysis. While MoSAIC-ReID achieves competitive performance on Market-1501 and DukeMTMC under the assumption that attribute annotations are available at test time, its primary value lies in providing a large-scale, quantitative study of attribute importance across intrinsic and extrinsic cues. Using generalized linear models, statistical tests, and feature-importance analyses, we reveal which attributes, such as clothing colors and intrinsic characteristics, contribute most strongly, while infrequent cues (e.g. accessories) have limited effect. This work offers a principled framework for interpretable ReID and highlights the requirements for integrating explicit semantic knowledge in practice. Code is available at https://github.com/psaltaath/MoSAIC-ReID

==> tables/experiments-duke.tex <==
\begin{table}[htbp]
\centering
\label{tab:duke_attributes}
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}cccccccccccc@{}}
\toprule
Backpack & Bag & Handbag & Hat & Boots & Shoe Color & Top & Gender & Down Color & Up Color & mAP & rank-1 \\
\midrule
\ding{52} & \ding{52} & \ding{52} & \ding{52} & \ding{52} & \ding{52} & \ding{52} & \ding{52} & \ding{52} & \ding{52} & \textbf{85.7} & \textbf{93.3} \\
\ding{52} & \ding{52} & \ding{52} & \ding{52} & \ding{52} & \ding{52} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & 83.7 & 92.0 \\
\ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{52} & \ding{56} & \ding{56} & \ding{52} & 83.1 & 91.9 \\
\ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{52} & \ding{52} & \ding{56} & \ding{56} & \ding{52} & \ding{56} & 83.7 & 92.2 \\
\ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{52} & \ding{56} & \ding{56} & 82.6 & 91.8 \\
\ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{52} & \ding{56} & \ding{56} & \ding{56} & 82.6 & 92.1 \\
\ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{52} & 82.9 & 92.1 \\
\ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{52} & \ding{56} & 83.0 & 91.9 \\
\ding{56} & \ding{56} & \ding{56} & \ding{52} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & 82.5 & 91.6 \\
\ding{52} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & 82.8 & 92.1 \\
\ding{56} & \ding{52} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & 82.6 & 91.8 \\
\ding{56} & \ding{56} & \ding{52} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & 82.6 & 92.2 \\
\ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{52} & \ding{56} & \ding{52} & \ding{52} & 83.5 & 92.0 \\
\ding{52} & \ding{52} & \ding{52} & \ding{52} & \ding{56} & \ding{56} & \ding{52} & \ding{56} & \ding{56} & \ding{52} & 83.6 & 92.3 \\
\ding{52} & \ding{52} & \ding{52} & \ding{52} & \ding{52} & \ding{52} & \ding{56} & \ding{56} & \ding{52} & \ding{52} & 84.3 & 92.3 \\
\ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{52} & \ding{52} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & 83.0 & 91.8 \\
\ding{52} & \ding{52} & \ding{52} & \ding{52} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & 83.4 & 92.3 \\
\ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{52} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & 82.5 & 91.6 \\
\ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{52} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & 82.6 & 91.9 \\
\ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \underline{82.6} & \underline{91.6} \\
\bottomrule
\end{tabular}%
}
\caption{Experimental results for DukeMTMC dataset}
\end{table}


==> tables/experiments-market.tex <==
\begin{table}[htbp]
\centering
\label{tab:market1501_attributes}
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}ccccccccccccccc@{}}
\toprule
Gender & Hair & Age & Hat & Backpack & Bag & Handbag & Up & Upcolour & Down & Downcolour & Clothes & mAP & rank-1 \\
\midrule
\ding{52} & \ding{52} & \ding{52} & \ding{52} & \ding{52} & \ding{52} & \ding{52} & \ding{52} & \ding{52} & \ding{52} & \ding{52} & \ding{52} & \textbf{95.5} & \textbf{97.9} \\
\ding{52} & \ding{52} & \ding{52} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & 90.8 & 96.2 \\
\ding{56} & \ding{56} & \ding{56} & \ding{52} & \ding{52} & \ding{52} & \ding{52} & \ding{52} & \ding{52} & \ding{52} & \ding{52} & \ding{52} & 94.6 & 97.6 \\
\ding{52} & \ding{52} & \ding{52} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{52} & \ding{52} & \ding{56} & \ding{56} & \ding{56} & 91.9 & 96.7 \\
\ding{52} & \ding{52} & \ding{52} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{52} & \ding{52} & \ding{52} & 92.7 & 97.5 \\
\ding{52} & \ding{52} & \ding{52} & \ding{52} & \ding{52} & \ding{52} & \ding{52} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & 92.4 & 96.6 \\
\ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{52} & \ding{52} & \ding{52} & 91.3 & 96.4 \\
\ding{56} & \ding{56} & \ding{56} & \ding{52} & \ding{52} & \ding{52} & \ding{52} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & 91.2 & 95.8 \\
\ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{52} & \ding{52} & \ding{56} & \ding{56} & \ding{56} & 90.7 & 95.6 \\
\ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{52} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & 89 & 95.2 \\
\ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{52} & \ding{56} & \ding{56} & \ding{56} & 90.3 & 95.3 \\
\ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{52} & \ding{56} & 90.6 & 95.6 \\
\ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{52} & \ding{56} & \ding{56} & 88.5 & 95.0 \\
\ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{52} & 88.9 & 95.1 \\
\ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{52} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & 89.6 & 95.2 \\
\ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{52} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & 89.2 & 94.8 \\
\ding{56} & \ding{56} & \ding{56} & \ding{52} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & 88.6 & 94.6 \\
\ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{52} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & 89.4 & 94.8 \\
\ding{56} & \ding{52} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & 89 & 95.1 \\
\ding{56} & \ding{56} & \ding{52} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & 89.8 & 95.4 \\
\ding{52} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & 88.5 & 94.6 \\
\ding{52} & \ding{52} & \ding{52} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{52} & \ding{52} & \ding{52} & \ding{52} & \ding{52} & 93.8 & 97.6 \\
\ding{52} & \ding{52} & \ding{52} & \ding{52} & \ding{52} & \ding{52} & \ding{52} & \ding{52} & \ding{52} & \ding{56} & \ding{56} & \ding{56} & 93.6 & 97.4 \\
\ding{52} & \ding{52} & \ding{52} & \ding{52} & \ding{52} & \ding{52} & \ding{52} & \ding{56} & \ding{56} & \ding{52} & \ding{52} & \ding{52} & 94.5 & 97.5 \\
\ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \ding{56} & \underline{89.6} & \underline{95.5} \\
\bottomrule
\end{tabular}%
}
\caption{Experimental results for Market1501 dataset}
\end{table}


==> tables/glm-duke.tex <==
\begin{table}
\label{tab:glm_results}
\resizebox{\linewidth}{!}{%
\begin{tabular}{lrrrrrr}
\toprule
 & Coef. & Std.Err. & z & P$>$$|$z$|$ & [0.025 & 0.975] \\
\midrule
Intercept & 82.405 & 0.078 & 1046.590 & 0.000 & 82.251 & 82.559 \\
backpack & 0.369 & 0.211 & 1.745 & 0.080 & -0.045 & 0.784 \\
bag & 0.169 & 0.211 & 0.801 & 0.422 & -0.245 & 0.584 \\
handbag & 0.169 & 0.211 & 0.801 & 0.422 & -0.245 & 0.584 \\
hat & 0.069 & 0.211 & 0.329 & 0.741 & -0.345 & 0.484 \\
boots & 0.323 & 0.186 & 1.734 & 0.082 & -0.042 & 0.688 \\
shoecolour & 0.223 & 0.186 & 1.197 & 0.231 & -0.142 & 0.588 \\
top & 0.306 & 0.166 & 1.841 & 0.065 & -0.019 & 0.632 \\
gender & 0.483 & 0.187 & 2.573 & 0.010 & 0.115 & 0.851 \\
downcolour & 0.604 & 0.150 & 4.027 & 0.000 & 0.310 & 0.898 \\
upcolour & 0.285 & 0.167 & 1.705 & 0.088 & -0.042 & 0.613 \\
\bottomrule
\end{tabular}%
}
\caption{GLM regression results on DukeMTMC}
\label{table-glm-duke}

\end{table}

==> tables/t-tests-duke.tex <==
\begin{table}
\label{tab:ttest_results}
\resizebox{\linewidth}{!}{%
\begin{tabular}{lrrrr}
\toprule
Feature & t-stat & p-value & Cohen's d & Significance \\
\midrule
backpack & -2.555 & 0.046 & 1.739 & * \\
bag & -2.340 & 0.061 & 1.613 &  \\
handbag & -2.340 & 0.061 & 1.613 &  \\
hat & -2.237 & 0.071 & 1.554 &  \\
boots & -2.088 & 0.086 & 1.443 &  \\
shoecolour & -1.998 & 0.097 & 1.391 &  \\
top & -1.300 & 0.255 & 0.967 &  \\
gender & -0.704 & 0.608 & 1.503 &  \\
downcolour & -2.451 & 0.064 & 1.926 &  \\
upcolour & -2.251 & 0.067 & 1.498 &  \\
\bottomrule
\end{tabular}%
}
\caption{t-Test Results for Attribute inclusion vs mAP on DukeMTMC dataset}
\end{table}



==> tables/t-tests-market.tex <==
\begin{table}
\label{tab:ttest_results}
\resizebox{\linewidth}{!}{%
\begin{tabular}{lrrrr}
\toprule
Feature & t-stat & p-value & Cohen's d & Significance \\
\midrule
gender & -3.298 & 0.006 & 1.509 & ** \\
hair & -3.549 & 0.003 & 1.590 & ** \\
age & -3.981 & 0.001 & 1.731 & ** \\
hat & -2.802 & 0.024 & 1.542 & * \\
backpack & -3.226 & 0.011 & 1.686 & * \\
bag & -3.341 & 0.009 & 1.724 & ** \\
handbag & -3.115 & 0.014 & 1.648 & * \\
up & -2.578 & 0.031 & 1.334 & * \\
upcolour & -3.206 & 0.010 & 1.542 & ** \\
down & -2.900 & 0.021 & 1.630 & * \\
downcolour & -4.203 & 0.002 & 2.073 & ** \\
clothes & -3.114 & 0.015 & 1.705 & * \\
\bottomrule
\end{tabular}%
}
\caption{t-Test Results for Attribute inclusion vs mAP on Market1501 dataset}
\end{table}
